Democratizing LEO Satellite Network Measurement

Low Earth Orbit (LEO) satellite networks are quickly gaining traction with promises of impressively low latency, high bandwidth, and global reach. However, the research community knows relatively little about their operation and performance in practice. The obscurity is largely due to the high barrier of entry for measuring LEO networks, which requires deploying specialized hardware or recruiting large numbers of satellite Internet customers. In this paper, we introduce HitchHiking, a methodology that democratizes global visibility into LEO satellite networks. HitchHiking builds on the observation that Internet-exposed services that use LEO Internet can reveal satellite network architecture and performance, bypassing the need for specialized hardware. We evaluate HitchHiking against ground truth measurements and prior methods, showing that it provides more coverage and accuracy. With HitchHiking, we complete the largest study to date of Starlink network latency, measuring over 2,400 users across 13 countries. We uncover unexpected patterns in latency that surface how LEO routing is more complex than previously understood. Finally, we conclude with recommendations for future research on LEO networks.

==> scraps.tex <==
\vspace{3pt}
\noindent
\textbf{Exposed Services.}\quad
Exposed services on the public Internet have been widely studied in a variety of contexts. 
Mirian et al. found over 60K publicly accessible and vulnerable ICS devices belonging to water controllers, power companies, medical facilities, and financial institutions~\cite{mirian2016internet}.
Kumar et al. studied publicly visible IoT devices in the home, and found that nearly half had a known vulnerability or weak password~\cite{kumar2019all}. 
Springall et al. studied publicly exposed FTP servers across the entire IPv4 address space and found that 1.1 million (8\%) FTP servers exposed content, a subset of which are shown to have been mistakenly configured~\cite{springall2016ftp}. 

% Vulnerable Internet services---especially on IoT devices~\cite{costin2014large}---are not just a hypothetical threat, and have led to the emergence of botnets~\cite{mirai,hunting,malecot2013carna}, distribution of malware~\cite{chen2009information}, and denial of service attacks~\cite{sisalem2006denial}.
% Researchers have shown that Internet-exposed devices can have been used to mount attacks to internal networks even when back authentication mechanisms are available~\cite{zdnetWhatsOnYourNetwork, albataineh2019iot, kumar2019all}.
% Attackers have even converted virtual vulnerabilities into physical attacks, causing the shut down a major gas pipeline~\cite{colonialPipeline} and electric grid~\cite{ukrainePowerGrid}.

\vspace{3pt}
\noindent
\textbf{Internet Measurement Vantage Points.}\quad
\todo{}
Although Internet scanning helps attackers find their target, it also helps researchers protect users and secure the Internet ecosystem. 
For example, Marczak et~al.\ used Internet-wide scans to identify spyware infrastructure~\cite{marczak2021candiru} and clients of cyber espionage~\cite{marczak2020running}.
Pearce et al. measured censorship and blocklisting through devices with global IPID counters~\cite{pearce2017augur, pearce2017global}.
Heninger et al. uncovered weaknesses in the Linux RNG through exposed IoT devices~\cite{heninger2012mining}.



%%%%%%%%%%%%%%%%CGNAT STory



% a non-consistent network assignment scheme, as we  describe below, contributes to the varying likelihood of a customer receiving either a public or private IP address. 

Traditionally, Starlink operated most similarly to a Carrier-Grade Network Address Translation (CGNAT) Internet Service Provider.
CGNAT is used to extend the capacity of ISP networks by sharing a small pool of public IP addresses among a large number of customers. 
Additionally, CGNAT improves security by hiding the internal IP addresses of devices behind a public IP address, making it difficult for attackers to target specific devices on the network.
Consequently, the majority of customer services were assigned a private IP address, thereby mitigating the number of publicly accessible services.

The lack of public IP addresses in a CGNAT network hindered remote access to devices, which caused inconveniences for some Starlink customers. 
Given some of the Starlink use cases, such as supporting remote sensors~\cite{reddit_remote}, this lack of easy remote access  led to a trove of online tutorials documenting the use of VPNs or bypassing Starlink routers to allow for remote access to their Starlink endpoints~\cite{cgnat_circumvantion,reddit_ddwrt}. 
%In fact, we see robust use of these remote access protocols for Starlink endpoints (Section~\ref{sec:characterize}).

However, starting from October 2021, users began unsolicitedly receiving public IP address from Starlink~\cite{reddit_starlink_1,reddit_starlink_2}.
Further complicating matters, users reporting being randomly switched to a public IP address and CGNAT~\cite{reddit_starlink_3}.
Thus, unbeknownst to users, previously private services (e.g., router login pages) suddenly, and without warning, became publicly exposed. 
Today, services in Starlink can become publicly accessible due to a variety of reasons, ranging from purposeful configuration by the customer to the random assignment of a public IP address.
%Our findings in Section ~\ref{sec:general_prevelance} are consistent with those reports. 

%These publicly exposed Starlink endpoints, form the basis of the analysis presented in this paper. We are in the process of disclosing these findings to Starlink.
%  But at times network changes can lead to services being exposed
% Customers want to access their starlink endpoints remotely. Being behind a CGNAT means people need to use VPN, PPTP
% Starlink also allows customers to replace Starlink router with own router.

% % For example, Starlink doesnt actually allow you to do this...but customers are doing it anyway. 
% Customers replacing Starlink router with their own:
% see commented out links
% %https://www.reddit.com/r/Starlink/comments/jqhoqz/starlink_app_works_fine_behind_own_router/?utm_source=share&utm_medium=ios_app&utm_name=iossmf



%%%%%%%%ONE WEB%%%%%%%%

%When predicting OneWeb latency, we use the same 500~mile \lv deployment to scan a OneWeb exposed service located on the Alaskan island of Saint Paul~\footnote{We confirm the location of the exposed service using WhoIs records, Censys Geolocation, and online sleuthing~\cite{fb_stpaul}}, at the building location of corporation that is testing OneWeb~\tcite{https://www.facebook.com/TanadgusixCorporation/posts/wednesday-february-23-2022dear-saint-paul-island-shareholderstdx-information-tec/2419970114805244/}. 





\subsection{Starlink User Ground Station Usage in the Wild}

\vspace{3pt}
\noindent
\textbf{Incoming Connections}\quad
1. Routing close to dish when client->dish? How often does this occur across geographies (e.g., make a cdf for the distance between geolocation of IP before starlink ASN (in traceroute) and PoP location).

Does this tell us that starlink so far for incoming connections is prioritizing terrestrial, and not ISL routing? 

\vspace{3pt}
\noindent
\textbf{Outgoing Connections}\quad
1.Routing Dish -> server shows that groundstation usage is not always the seemingly closes to the dish. Make same CDF as Incoming connections for Dish->server traceroutes.

Gien the total RTT< does it look ISLs are being used? 




% \subsection{Performance Enhancement Proxies}
% PEP-link is a performance enhancement proxy which, among many features, provides a ``hot fail-over,'' in which users are able to fallback to standard cellular connection when Starlink faces an outage cut off. 
% We compare outage (i.e., the absence of at least 2 response packet when measuring RTT ) frequency and duration between peplink and non-peplink customers.
% We find noticeable differences when using peplink. 


% While in all but one POP peplink users never experience longer than a 15~second outage, in over 50\% of POP locations non-peplink users experience outages lasting at least 20~seconds. 
% In at least two POP locations (Nigeria and Columbia), non-peplink users experience a near 100~second outage, . 
% Nevertheless, outages constitute less than 1\% of all measurements across all POPs, thereby not soliciting a dire need for peplink outage protection.  

==> service-eco.tex <==
\section{Identifying Measurable Endpoints in LEO Networks}
\todo{Liz is working on this...}

To measure real-world LEO satellite network performance, \lhh needs reachable endpoints (e.g., servers, routers) that traverse a LEO satellite link.
In this section, we observe that there exist over 2,000 uniquely-identified hosts on the public Internet across multiple LEO satellite providers (e.g., Starlink, Oneweb) that can be candidates for \lhh measurement. 
Exposed services are geographically wide-spread across at least 20~countries and \TK cities, providing a worldwide pool of measurable endpoints. 
\todo{finish intro}

\subsection{Methodology}

To find Internet-exposed satellite endpoints we use Censys~\cite{censys15}, a public Internet device search engine. 
Censys performs continual scans of the full IPv4 address space and known IPv6 addresses (e.g., IPv6 address that appear in the Certificate Transparency Logs) on approximately 3,500~TCP and UDP ports. 
Censys then attempts to detect L7 protocol and complete an L7 handshake, when possible.
We note that our study is limited to only standardized Internet protocols that Censys is able to detect and may miss equipment that runs proprietary configurations; Censys does not currently scan any satellite-specific ports or protocols.

We specifically search for customer-exposed services in LEO satellite networks by searching for autonomous systems that belong to LEO satellite networks, including SpaceX-Starlink (ASN\,14593), OneWeb (ASN\,800), \TK .
\todo{which ones we choose and why}
In this section, we a present a breakdown of the data that was collected on May \TK, 2023.
Since it is likely that some services in a LEO autonomous system may not entirely (if at all) rely on a LEO satellite link, we discuss throughout this section and Section~\TK additional filtering steps to ensure end-points are very-likely connected over LEO satellite link.

\vspace{3pt}
\noindent
\textbf{Ethical Considerations.}\quad
Our study relies on open data published by Censys. 
To reduce the impact of scanning, we do not perform any additional Internet-wide scans. 
During the course of our investigation, we never attempt to login to or access any non-public data. 
While our search criteria can be used to uncover devices, these criteria are not difficult to uncover. Simply searching \texttt{starlink} on Censys uncovers terminals and other criteria are discussed openly online.
In our work we find multiple instances of sensitive data exposed by governments and other organizations. 
We are in the process of disclosing exposed access points to their owners.


\subsection{Exposed Services Are Geographically Widespread}

\input{tables/TopLocations.tex}

Starlink services are widespread across different cities and countries. 
To obtain an approximate geographic location of exposed services, we (1) query the domain name for each service's IP (e.g., customer.atlagax1.pop.starlinkisp.net) (2) use the geographic location specified in the domain name (e.g., atlagax) to map~\cite{reddit_mapping} to a geographic location (e.g., Atlanta, Georgia). 
We map all IPs to 15 \TK  unique points of presence (i.e., cities) across \TK 9~unique countries and present the distribution of mappings in Table~\ref{tab:topLocations}. \todo{update table w/ new data}
While the vast majority (80\%) of exposed IPs reside in the US, there exists a long-tail of other geographic locations including Australia (10\%), Nigeria (\TK\%), Japan (\TK\%) and Columbia (\TK\%). 


To determine the geographic location of OneWeb services, we capitalize on an observation: OneWeb enterprise customers are listed as the registrant of One Web IP addresses in the whois database.
Thus, we use the location of the registrant to determine the likely location of the service. 
Unlike Starlink, the majority of OneWeb expoesed services are located in Northern regions, including Alaska (add \TK). 
\todo{add one web to table}



\subsection{How Services Become Exposed}

To configure a service to be publicly accessible over the Internet, the service requires a publicly routeable IP address. 
We find that different customers must jump through different hoops to expose services over LEO satellite networks.  

For example, while all Starlink customers on the ``Business'' plan\footnote{\url{https://www.starlink.com/business}} can request both a publicly routeable IPv4 and IPv6 address,  customers on all other plans can only request publicly routeable IPv6 addresses. 
Nevertheless, there have been cases where non-business Starlink users unsolicitedly receive public IPv4 addresses from Starlink~\cite{reddit_starlink_1,reddit_starlink_2,reddit_starlink_3}.  
The current generation of Starlink routers do not allow port-forwarding, requiring users to use their own routers to host publicly accessible services~\cite{reddit_ddwrt}. 

Since OneWeb only caters to enterprise clients and governments, their exists little public information regarding the specifics of their networking solutions. 
Nevertheless, their dedication to custom solutions~\tcite{}, likely includes providing public IP addresses and port-forwarding ability to clients. 


%not dicussing VPN ref{cgnat_circumvantion} since that wont appear in the address space we are studying


% However, starting from October 2021, users began unsolicitedly receiving public IP address from Starlink~\cite{reddit_starlink_1,reddit_starlink_2}.
% Further complicating matters, users reporting being randomly switched to a public IP address and CGNAT~\cite{reddit_starlink_3}.



\subsection{What services do customers expose?}

% \todo{integrate: In fact, we see robust use of these remote access protocols for Starlink endpoints (Section~\ref{sec:characterize}).}

Customers expose a wide variety of applications across the Starlink network. 
We identify a total of \TK 1544 exposed services across \TK 724 unique IPs,\TK  222 unique ports, and \TK 30~application layer protocols. 
We present the top 10~most common application layer protocols in Table~\ref{tab:topServices}.
Over half (55\%) of exposed services host an HTTP service.
The majority (58\%) of the exposed HTTP services host login pages (i.e., return a response that prompts the client to enter a username and password). 
A quarter of the login pages belong to Sonicwall devices, which have historically been vulnerable to attacks~\cite{sonicwalljan,sonicwalljuly}.
Occasionally, login pages that appear to require credentials practice poor security; we encounter multiple login pages for a Cisco networked service~\cite{meraki} which explicitly provides the format for a username and states that, although prompted, no password is required.
Nearly 41\% of services across all protocols host a login page. 

HTTP applications that do not expose login pages are often even more vulnerable, exposing sensitive network or critical infrastructure data.
Upon a manual investigation of the remaining HTTP services, we identify multiple passwordless exposed data panels.
For example, we find a NetGear control panel that monitors local network usage, including bandwidth usage and localhost names. 
The control panel displays an SSID that reveals the owner to be a state fire department and localhost names that reveal the names of device users~\cite{imc22hostnames}.
Upon googling the names of the device users, we confirm that they are firefighters who work for that fire department. 
%https://98.97.123.121:8009
We also identify a weather panel that monitors the temperature, barometric pressure, and humidity of its location, also belonging to a government entity. 
%http://98.97.120.237:8080


Customers also expose a longtail of many different unique applications. 
For example, 6\% of exposed services host SSH.
%While the most popular vendor to host SSH is OpenBSD,
Routers and appliances vendors often expose SSH, including Cisco (24\% of all SSH services), MikroTik (18\%), Dropbear (14\%) and  Sonicwall (8\%).
A small fraction (10\%) of exposed services are uncommon and, consequently, not fingerprinted by Censys (denoted by the UNKNOWN protocol in Table~\ref{tab:topServices}). 
We manually investigate the applications and find that 20\% of them belong to Peplink~\cite{pep} a customer deployed performance enhancing proxy tailored towards Starlink. 
In Figure~\ref{tab:topVendors} we present the top 10~most common vendors, which include middlebox vendors such as Sonic-Wall, GFI, Hikvision, and Cisco. 
Across all applications, vendors that produce middlebox appliances (e.g., routers, firewalls) expose the most services.

%630 login pages, with the vast majority being hosted on HTTP. 

%\textbf{Fortiguard.}

%\textbf{NTP.}

%\textbf{OpenVPN.}
%Port 1194 hosting openVPN,
Exposed services in Starlink inhabit both assigned and unassigned ports. 
Prior work has found that, across the public IPv4 space, services more often than not live on uncommon ports~\cite{lzr}; we find roughly half of exposed satellite services run on their assigned port. 
Amongst the top 10~most common ports that host services, only three are unassigned/uncommon: ports~4443 (3\% of services), 8443 (2\%), and 32015 (2\%). 
Firewalls and other IoT appliances dominate uncommon ports, which is consistent with prior work~\cite{lzr}.
For example, 76\% of services on port 4433 belong to Fortiguard products. 
A longtail of appliances inhabit port~8443 such as SonicWall equipment~\cite{sonicwall}, DropbearSSH~\cite{sshdropbear}, Hikvision~\cite{hikvision}, and Cradlepoint~\cite{cradlepoint}.

%People are hiding TLS services on less common ports: 4433 (76\% is Fortiguard) , 
%8443 Longtail, but dominated also by IoT (9	SonicWall , 3 Dropbear, Hikvision, Cradlepoint, etc)
% 7	lighttpd
% 3	Dropbear SSH Project
% 3	Fortinet
% 3	Microsoft
% 3	redhat
% 2	Cradlepoint
% 2	Kubernetes
% 2	OpenBSD
% 2	microsoft
% 1	3CX
% 1	Hikvision
% 1	Ubiquiti
% 1	Ubuntu
% 1	WatchGuard
% 1	mod_wsgi
% 1	nginx


\subsection{Who is exposing services?}

Services are exposed by a wide range of entities: individual customers and 
prominent organizations, including governments and companies. 
To fingerprint the owners of services, we analyze the names in all 392~TLS certificates. 
Most alarmingly, we identify three TLS certificates registered to a `.gov' domain: 
the first is hosted by the US government and appears to expose a weather radar near the south pole,
the second is hosted by a city government in the US and exposes a SonicWall login page,
and the third is hosted by the Australian government and appears to expose mail servers.

We identify 23 TLS certificates that belong to a company.
For example, two companies are in the maritime industry---an industry that makes popular use of satellite Internet~\cite{pavur2020tale}---including a prominent cruise ship company that exposed multiple login pages to Fortigate firewalls. %virgin voyages
Other companies include a winery, two golf clubs, an energy company, and a commercial farm. 
The most common shared TLS certificate amongst all exposed services belongs to the peplink (customer deployed performance enhancing proxies), which across all customers exposes 98 login pages. 



% \subsection{Ethical Considerations}
% Exposed services are often abused by attackers~\tcite{}
% - no abuse by attackers; although unfortunately attackers have already noticed and claimed to have exploited user terminals. 
% Whenever we find services that appear undoubtedly vulnerable, we reach out to any identifiable owners. 
% As the satellite academic community continues to grow, we will continue to work with other researchers to develop guidelines that simultaneously minimizes vulnerable exposed services and maximizes our opportunity to use this diverse set of vantage points. 


\subsection{Summary}




==> tables/TopPorts.tex <==

\begin{table}[t]
%\centering
\centering
\begin{tabular}{lll}
\toprule
Port   & \# Services & \\
\midrule
	443 /HTTPS & 334 \\
	80 /HTTP & 209 \\
 	22/SSH & 63 \\ 
541 /FORTIGUARD & 63	\\
123/NTP & 39	 \\
	4433/UNASSIGNED & 38 \\
	8443/UNASSIGNED & 34 \\
1194/OPENVPN & 28	 \\
 	32015/UNASSIGNED & 27 \\
 500/IKE & 22	 \\
\midrule
Total &  \TK /1544  (\TK \%)\\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\textbf{Top 10 Exposed Ports}---%
\textnormal{HTTP....}}
\label{tab:topPorts}
%\vspace{-15pt}
\end{table}





==> tables/TopServices.tex <==
\begin{table}[t]
%\centering
\centering
\begin{tabular}{lll}
\toprule
Application   & \# Services & \\
\midrule
HTTP & 848 \\
UNKNOWN & 152\\
SSH  & 84 \\
FORTIGUARD  & 59 \\
NTP & 39	\\
OPENVPN & 26 \\
IKE & 22\\
PPTP &19\\
RTSP & 17\\
DNS & 12 \\
\midrule
Total &  1278/1544 (83\%)\\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\textbf{Top 10 Exposed Applications}---%
\textnormal{Starlink customers expose a longtail of different applications, with HTTP pages being by far the most popular. }}
\label{tab:topServices}
%\vspace{-15pt}
\end{table}



% Jan 13:
% 848	HTTP
% 152	
% 84	SSH
% 59	FORTIGUARD
% 39	NTP
% 26	OPENVPN
% 22	IKE
% 19	PPTP
% 17	RTSP
% 12	DNS
% 11	MIKROTIK_BW
% 9	FORTIGATE
% 8	RDP
% 8	TELNET
% 7	FTP
% 7	SNMP
% 6	VNC
% 4	SMTP
% 3	ANYCONNECT
% 3	MQTT


% HTTP: 
% 165	nginx
% 119	SonicWall
% 85	Apache
% 40	GFI
% 39	OpenBSD
% 36	Hikvision
% 30	Microsoft
% 28	lighttpd
% 20	Fortinet
% 15	Ubiquiti

% SSH:
% 46	OpenBSD
% 20	Cisco
% 20	nginx
% 16	Debian
% 15	MikroTik
% 12	Dropbear SSH Project
% 10	Ubiquiti
% 9	Apache
% 9	Cradlepoint
% 9	Ubuntu
% 9	lighttpd
% 8	PHP
% 7	SonicWall
% 4	OpenResty
% 3	Microsoft
% 2	Linksys
% 2	cisco
% 2	freebsd
% 1	CaddyServer
% 1	CherryPy

==> tables/TopVendors.tex <==

\begin{table}[t]
%\centering
\centering
\begin{tabular}{lll}
\toprule
Vendor   & \# Services & \\
\midrule
	nginx & 165 \\
	SonicWall & 119 \\
 	Apache & 85 \\ 
  Microsoft & 54 \\
 OpenBSD & 46	\\
GFI & 40	 \\
 Hikvision & 36 \\
Lighttpd& 28	 \\
Cisco & 25 \\
Fortinet & 21	 \\
\midrule
Total &  598/1544  (40\%)\\
\bottomrule
\end{tabular}
\vspace{8pt}
\caption{\textbf{Top 10 Exposed Vendors}---%
\textnormal{Vendors that provide routers and middleboxes often house exposed services.  }}
\label{tab:topVendors}
%\vspace{-15pt}
\end{table}


%Vendors:
%165	nginx
%119	SonicWall
%85	Apache
%46	OpenBSD
%40	GFI
%36	Hikvision
%32	Microsoft
%28	lighttpd
%25	Cisco
%22	microsoft



%Products:
%165	nginx
%128	HTTP
%119	SonicOS
%91	linux
%82	HTTPD
%46	OpenSSH
%40	Kerio Control
%36	Hikvision Web Server
%36	Linux
%28	lighttpd


==> tables/search.tex <==
\begin{table}
\begin{center}
\begin{tabular}{ll} 
\toprule
Satellite Endpoint & Search Heuristic \\ \midrule
Starlink & autonomous\_system: 14593 \\
\midrule
VIASAT & autonomous\_system in (7155, 16491, 40306, \\
&  40311,46536 209945,262364,210027,29242, \\
& 40310,40313) and \\
& dns.reverse\_dns.names: *.cust.exede.net \\ 
\midrule
Satellite Modems Across Vendors & ``Satellite Modem'' in HTML Title \\
\bottomrule
\end{tabular}
\caption{Satellite Services Search Criteria}
\label{tab:search_crit}
\end{center}
\end{table}
